Generating High-Resolution Regional Precipitation Using Conditional Diffusion Model

Climate downscaling is a crucial technique within climate research, serving to project low-resolution (LR) climate data to higher resolutions (HR). Previous research has demonstrated the effectiveness of deep learning for downscaling tasks. However, most deep learning models for climate downscaling may not perform optimally for high scaling factors (i.e., 4x, 8x) due to their limited ability to capture the intricate details required for generating HR climate data. Furthermore, climate data behaves differently from image data, necessitating a nuanced approach when employing deep generative models. In response to these challenges, this paper presents a deep generative model for downscaling climate data, specifically precipitation on a regional scale. We employ a denoising diffusion probabilistic model (DDPM) conditioned on multiple LR climate variables. The proposed model is evaluated using precipitation data from the Community Earth System Model (CESM) v1.2.2 simulation. Our results demonstrate significant improvements over existing baselines, underscoring the effectiveness of the conditional diffusion model in downscaling climate data.

==> 7_kaia_summary.tex <==
\onecolumn
	\begin{center}
		\section*{Summary of this paper}	
		\setcounter{subsection}{0}
	\end{center}
\noindent\fbox{
    \parbox{\textwidth}{
    	\begin{quote}
		\subsection{Problem Setup}
		% \vspace{0.5\baselineskip}
        Our objective is to produce high-resolution (HR) regional climate data from low-resolution (LR) global climate data, a process referred to as “climate downscaling” (a term that refers to projecting global scale climate data, down onto regional scales). Previous approaches limitation: most deep learning models for climate downscaling may not perform optimally for high scaling factors (i.e., 4x, 8x) due to their limited ability to capture the intricate details required for generating HR climate data. Furthermore, climate data behaves differently from image data, necessitating a nuanced approach when employing deep generative models.
        
		\subsection{Novelty}
		% \vspace{0.5\baselineskip}
        \textbf{Dataset}: We employed 20 years (N = 20 × 365 = 7300) of HR data from a global climate HR simulation conducted with the fully-coupled, global circulation climate model CESM version 1.2.2. This data represents daily means over the North America region. \textbf{Method}: Implementing careful approach when using climate variables as the model's input and output channels as opposed to the practices within the field of computer vision. \textbf{Impact}: It highlights the important of careful approach to the design the inter-channel and intra-channel relationships in downscaling climate variables, especially in employing denoising model which can be a potential for downscaling climate data from a wide range of climate model simulations.

  
		\subsection{Algorithms}
        The proposed algorithm is based on denoising diffusion probabilistic model (DDPM) conditioned on low-resolution (LR) climate variables, yielding a single target climate variable, as opposed to generating an equivalent number of variables as the model input (similar to image channels in computer vision applications). The process can be mainly divided in 2 steps. The firs step is training the denoising model by using multiple LR climate variables as the condition to the model. The model objective is denoising the target HR climate variable (backward diffusion process) by iteratively predicting the noise added in pre-defined forward diffusion process. The second step is the inference, where the model will generate HR climate variables from simple data distribution, i.e. gaussian distribution, by iteratively improving the generation guided by corresponding LR climate data as the condition.
		\subsection{Experiments}
        \textbf{Data:} 
        Climate variables from a global climate HR simulation conducted with the fully-coupled, global circulation climate model CESM version 1.2.2. The HR data from the climate simulation represents daily means over the North America region for 20 years (N = 20 × 365 = 7300). We split the data into 5300 datapoints for the training, 500 for the validation, and 1500 for the test data. The HR data has a resolution of 213×321, with each pixel representing an approximate grid resolution of 25 kilometers. To generate LR data, we apply bicubic interpolation to convert the HR data into a coarser resolution, i.e. into 4x and 8x scale factors.
        \textbf{Evaluation:}
        We "downscale" 1500 data points extracted from the CESM v1.2.2 climate model. Performance assessment is carried out by calculating the root mean squared error (RMSE) through a comparison between the model’s output and the high-resolution ground truth data over 4x and 8x scale factors. Our evaluation includes a comparison with traditional techniques, specifically bilinear and bicubic interpolation, alongside convolution network models like SRResNet and U-Net. 
        \textbf{Results:}
        The experiment results show substantial improvements in the performance compared to existing baselines, indicating the effectiveness of the conditional diffusion model in downscaling climate data. Moreover, we experiment with how the number of climate variables used in the model affects the performance, i.e. 3 input channels-3 output channels versus 3 input channels-1 output channels, which can be seen visually. This highlights the need for a careful approach when employing deep learning in climate variables.
        
		\end{quote}
    }
}
\thispagestyle{empty}
